Q-learning for POMDP: An application to learning locomotion gaits

This paper presents a Q-learning framework for learning optimal locomotion gaits in robotic systems modeled as coupled rigid bodies. Inspired by prevalence of periodic gaits in bio-locomotion, an open loop periodic input is assumed to (say) affect a nominal gait. The learning problem is to learn a new (modified) gait by using only partial noisy measurements of the state. The objective of learning is to maximize a given reward modeled as an objective function in optimal control settings. The proposed control architecture has three main components: (i) Phase modeling of dynamics by a single phase variable; (ii) A coupled oscillator feedback particle filter to represent the posterior distribution of the phase conditioned in the sensory measurements; and (iii) A Q-learning algorithm to learn the approximate optimal control law. The architecture is illustrated with the aid of a planar two-body system. The performance of the learning is demonstrated in a simulation environment.

==> _definitions.tex <==
%%%spm macros %%%
\def\qed{\hspace*{\fill}~\IEEEQED\par\endtrivlist\unskip}%\mbox{\rule[0pt]{1.3ex}{1.3ex}}}
\def\tilW{\widetilde W}
\def\tilZ{\widetilde Z}
\def\hap{\hat{p}}
\def\haU{\widehat{U}}
\def\ddx{\frac{\ud}{\ud x}}
\def\ddt{\frac{\ud}{\ud t}}
\def\Re{\mathbb{R}}
\def\R{\mathbb{R}}
\def\T{[0,2\pi]}
\def\KL{\,\text{\rm KL}}
\def\argmin{\mathop{\text{\rm arg\,min}}}
\def\ind{\text{\rm\large 1}}
\def\varble{\,\cdot\,}
%This is p_n: \def\pxzn{p_{\text{\tiny$ X| Z^n$}}}
\def\pxz{p_{\text{\tiny$ X| Z$}}}
\def\pzx{p_{\text{\tiny$ Z | X$}}}
\def\pdzx{p_{\text{\tiny $ \ud Z | X$}}}
\def\pz{p_{\text{\tiny$Z$}}}
\def\pdz{p_{\text{\tiny$\ud Z$}}}
\def\ps{p_{\text{\tiny$S$}}}
\def\tilh{\tilde h}
\def\tilz{\tilde z}
\def\tilp{\tilde p}
\def\Hil{\mathbf H}
\def\Ltwo{\mathbf{L}^2}
\newcommand{\Real}{\mathbb R}
\def\ddx{\frac{\ud}{\ud x}}
\def\ddt{\frac{\ud}{\ud t}}
\def\frakp{\mathfrak{p}}
\def\frakh{\mathfrak{h}}
\def\frakz{\mathfrak{z}}
\def\solp{\frakp}
\def\solh{\frakh}
\def\solz{\frakz}
\def\varble{\,\cdot\,}
\def\bfInov{\bfmath{I}}
\def\Inov{I} %So we can change symbol easily later
\def\pop{\hbox{\tiny (POP)}}
\def\Lemma#1{Lemma~\ref{#1}}
\def\Proposition#1{Prop.~\ref{#1}}
\def\Theorem#1{Thm.~\ref{#1}}
\def\Corollary#1{Cor.~\ref{#1}}
\def\Sec#1{Sec.~\ref{#1}}
\def\Fig#1{Fig.~\ref{#1}}
\def\Appendix#1{Appendix.~\ref{#1}}
\def\notes#1{\marginpar{\tiny #1}\typeout{Notes!
Notes!
Notes!
}}
\renewcommand{\notes}[1]{\typeout{notes!}}
\def\FRAC#1#2#3{\genfrac{}{}{}{#1}{#2}{#3}}
\def\half{{\mathchoice{\FRAC{1}{1}{2}}%
{\FRAC{2}{1}{2}}%
{\FRAC{3}{1}{2}}%
{\FRAC{4}{1}{2}}}}
\def\prrr{{\cal T}}
\def\gen{{\cal D}}
\def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}
\def\ind{\bbbone}
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\tr}{\mbox{tr}}
\def\posRe{\field{R}_+}
\def\Re{\field{R}}
\def\k{{\sf K}}
\def\Co{\field{C}}
\def\Sec#1{Sec.~\ref{#1}}
%\def \eqdef {\mathrel {\mathop {=\joinrel=}\limits^{def}}}
\def\eqdef{\mathrel{:=}}
\def\defeq{\mathrel{=:}}
\def\transpose{{\hbox{\rm\tiny T}}}
\def\clB{{\cal B}}
\def\clE{{\cal E}}
\def\clL{{\cal L}}
\def\clP{{\cal P}}
\def\clZ{{\cal Z}}
\def\clZd{{\cal Z}^{{}\, \hbox{\tiny $\blacksquare$}}}
\def\clW{{\cal W}}
\def\Sec#1{Sec~\ref{#1}}
\def\bfmath#1{{\mathchoice{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$\scriptstyle#1$}}%
{\mbox{\boldmath$\scriptscriptstyle#1$}}}}
\def\bfInov{\bfmath{I}}
\def\Inov{I} %So we can change symbol easily later
\def\bfmX{\bfmath{X}}
\def\bfmZ{\bfmath{Z}}
\def\bfmU{\bfmath{U}}
\def\bfxi{\bfmath{xi}}


\newcommand{\img}{\text{Im}}
\newcommand{\barC}{\bar{C}}
\newcommand{\barc}{\bar{c}}
% \def\E{\text{E}}
\def\E{{\sf E}}
\def\Expect{{\sf E}}
\newcommand{\avgT}{\lim_{T\to\infty}\frac{1}{T}\!\!\!\int_0^T}
\newcommand{\avgTt}{\lim_{T\to\infty}\frac{1}{T}\!\!\!\int_t^T}
\def\intsw{\int_{\Omega}\!\int_0^{2\pi}}
\newcommand{\avgNni}{\frac{1}{N}\sum_{j\neq i}^N}
\newcommand{\avgN}{\frac{1}{N}\sum_{j=1}^N}
\newcommand{\Oscr}{\mathcal O}
\newcommand{\Lscr}{\mathcal L}
\newcommand{\dtheta}{\theta\theta}
\newcommand{\ptheta}{\partial_{\theta}}
\newcommand{\pthetaB}{\partial^2_{\dtheta}}
\newcommand{\pt}{\partial_{t}}
\newcommand{\zero}{\mathbf{0}}
\def\clC{{\cal C}}
\def\clX{{\cal X}}
\def\Prob{{\sf P}}
\def\Probsub{{\sf P\! }}
\def\Expect{{\sf E}}
\def\state{{\sf X}}
\def\spm#1{\notes{\textcolor{blue}{SPM: #1}}}
\def\pgm#1{\notes{\textcolor{blue}{PGM: #1}}}
\def\akt#1{\notes{\textcolor{blue}{akt: #1}}}
\def\wham#1{\smallbreak\noindent\textbf{\textit{#1}}}
\newcommand{\vu}{\vec{u}}
\newcommand{\ith}{i^\text{th}}
\newcommand{\jth}{j^\text{th}}
\def\hT{h^{(T)}}
\newcommand{\kth}{k^\text{th}}
\newcommand{\rth}{r^\text{th}}
\newcommand{\mth}{m^\text{th}}
\newcommand{\nth}{n^\text{th}}
\newcommand{\indi}{ {\small i} }
\newcommand{\indj}{ {\small j} }
\newcommand{\indm}{{\small m}}
%\newcommand{\indn}{{\small n}}
%\def\Lscr{\mathcal{L}}
\def\Lscr{\mathcal{Z}}
\def\Mscr{\mathcal{M}}
%\def\Nscr{\mathcal{N}}
%\def\Pscr{\mathcal{P}}
\def\Nscr{\mathcal{M}}
\def\Pscr{\Pi}
\def\Sscr{\mathcal{S}}
\def\R{\mathbb{R}}
\def\ie{i.e.\,}
\def\Fig#1{Fig.~\ref{#1}}
\def\Sec#1{Sec.~\ref{#1}}
\def\Subsec#1{Sec.~\ref{#1}}
\def\UZ{\underline{\mathcal{Z}}}
\def\UY{\underline{\mathcal{Y}}}
\def\uX{\underline{X}}
\def\uY{\underline{Y}}
\def\uZ{\underline{Z}}
\def\ua{\underline{\alpha}}
\def\uA{\underline{A}}
\def\upi{\underline{\pi}}
\def\ugamma{\underline{\gamma}}
\def\P{{\sf P}}
\def\Inov{I}
\def\ddx{\frac{\ud}{\ud x}}
\def\IEEEQEDclosed{\mbox{\rule[0pt]{1.3ex}{1.3ex}}}
\def\qed{\nobreak\hfill\IEEEQEDclosed}
%\def\M{\mathfrak{\bar{m}}}
%\def\N{\mathfrak{\bar{n}}}
\def\M{M}
\def\N{M}
\def\S{O}
\def\cth{c^\text{th}}
\def\lth{l^\text{th}}
\newcommand{\indicator}[1]{\mathbf{1}_{\left[ {#1} \right] }}
\newcommand{\cov}{\text{Cov}}



\newcommand{\pmat}[1]{\begin{pmatrix}#1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix}#1 \end{bmatrix}}


\newcommand{\vX}{X}
\newcommand{\Pos}{P}
\newcommand{\bearing}{h}
\newcommand{\bearingMean}{\hat{h}}
\newcommand{\Obs}{Z}
\newcommand{\Permm}[1]{\Pscr_{#1}}
\newcommand{\filtration}{\UZ}
\newcommand{\ProbAsso}{\beta}
\newcommand{\ProbPerm}{\gamma}
\newcommand{\assoc}[2]{#1 \equiv #2}
\newcommand{\particleX}{X}
\newcommand{\approxControlGain}{\tilde{\v}}
\newcommand{\innov}{I}
\newcommand{\expect}{ {\sf E} }
\newcommand{\velx}{\dot{x}}
\newcommand{\vely}{\dot{y}}
\def\clZ{{\cal Z}}
\def\varble{\,\cdot\,}

\def\eqdef{\mathrel{:=}}

%\newcommand{}{def}
%\newcounter{rmnum}
%\newenvironment{romannum}{\begin{list}{{\upshape (\roman{rmnum})}}{\usecounter{rmnum}
%\addtolength{\leftmargin}{-5pt}
%\setlength{\rightmargin}{4pt}
%}}{\end{list}}



% \def\RevComment#1#2{%
\newcommand{\RevComment}[3][Green]{
{\color{#1}{#2}}%
\marginpar{%
    \begin{flushleft}
	\tiny\color{#1}{#3}
    \end{flushleft}
}%
}
\newcommand{\RevChg}[2]{%
%{\color{red}{\sout{#1}}}% \xout
{\color{blue}{\uwave{#2}}}%
}
\newcommand{\RevDel}[1]{%
{\color{red}{\sout{#1}}}
}


%
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

\newcommand{\ali}[1]{\begin{align}#1\end{align}}
\def\prechi{\psi}

\def\beq{\begin{eqnarray}} 
\def\bc{\begin{center}} 
\def\be{\begin{enumerate}}
\def\bi{\begin{itemize}} 
\def\bs{\begin{small}}
\def\bS{\begin{slide}}
\def\ec{\end{center}} 
\def\ee{\end{enumerate}}
\def\ei{\end{itemize}}
\def\es{\end{small}}
\def\eS{\end{slide}}
\def\eeq{\end{eqnarray}}
\def\Xhat{\hat{X}}
\def\Yhat{\hat{Y}}
\def\Zhat{\hat{Z}}
\def\hah{\hat{h}}
\def\haphi{\hat{\phi}}
\def\hap{\hat{p}}
\def\hah{\hat{h}}
\def\haU{\widehat{U}}
\def\J{{\sf J}}
\def\Jstar{J^*}  %I didn't like a simple "J" -spm
\def\belief{\beta}

\def\bfbelief{\bfmath{\beta}}
\newcommand{\newP}[1]{\medskip\noindent{\bf #1:}}
\newcommand{\Rn}{\mathbb{R}^n}
\newcommand{\px}{\frac{\partial}{\partial x}}
\newcommand{\ppt}{\frac{\partial}{\partial t}}
\newcommand{\pp}[1]{\frac{\partial}{\partial #1}}
\newcommand{\pxx}{\frac{\partial^2}{\partial x^2}}
\newcommand{\diver}{\nabla \cdot}
\newcommand{\trace}{\text{Tr}}

\newcommand{\PP}{{\sf P}}
\newcommand{\mean}{\hat{X}}
\newcommand{\ud}{\,\mathrm{d}}
\newcommand{\NGs}{N}

\def\Re{\mathbb{R}}
\def\E{{\sf E}}
\def\KL{\,\text{\rm KL}}
\def\argmin{\mathop{\text{\rm arg\,min}}}
\def\argmax{\mathop{\text{\rm arg\,max}}}
\def\ind{\text{\rm\large 1}}
\def\varble{\,\cdot\,}

%This is p_n: \def\pxzn{p_{\text{\tiny$ X| Z^n$}}}
\def\pxz{p_{\text{\tiny$ X| Z$}}}
\def\pzx{p_{\text{\tiny$ Z | X$}}}
\def\pdzx{p_{\text{\tiny $ \ud Z | X$}}}
\def\pz{p_{\text{\tiny$Z$}}}
\def\pdz{p_{\text{\tiny$\ud Z$}}}
\def\ps{p_{\text{\tiny$S$}}}

\def\clY{{\cal Y}}

%%%

\def\Sec#1{Sec.~\ref{#1}}
\def\Thm#1{Thm.~\ref{#1}}
\def\Prop#1{Prop.~\ref{#1}}

\def\smopot{{\cal G}}

\def\bfmath#1{{\mathchoice{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$#1$}}%
{\mbox{\boldmath$\scriptstyle#1$}}%
{\mbox{\boldmath$\scriptscriptstyle#1$}}}}

\def\bfInov{\bfmath{I}}
\def\Inov{I} %So we can change symbol easily later

\def\bfPhi{\bfmath{\Phi}}
\def\bfmX{\bfmath{X}}
\def\bfmZ{\bfmath{Z}}
\def\bfmU{\bfmath{U}}
\def\bfmW{\bfmath{W}}
\def\bfxi{\bfmath{xi}}

\def\Expect{{\sf E}}

\def\sTriangle{\hbo x{\small $\triangle$}}


\def\clB{{\cal B}}
\def\clD{{\cal D}}
\def\clE{{\cal E}}
\def\clJ{{\cal J}}
\def\clL{{\cal L}}
\def\clP{{\cal P}}
\def\clZ{{\cal Z}}
\def\clZd{{\cal Z}^{{}\, \hbox{\tiny $\blacksquare$}}}
\def\w{{\sf \Omega}}%Wong-Zakai correction term

\def\clW{{\cal W}}

\def\haphi{\hat{\phi}}
\def\hap{\hat{p}}
\def\hah{\hat{h}}
\def\haU{\widehat{U}}
\newcommand{\dthet}{\dot{q}}
\newcommand{\cm}{_{\text{\tiny CM}}}
\newcommand{\JJ}{I_{(q)}}
\newcommand{\CN}{C^{(n)}}
\newcommand{\CT}{C^{(t)}}
\newcommand{\TT}{_{t}}
\newcommand{\CC}{\mathsf{R}}
\newcommand{\fgen}{f^{\text{gen}}}
\newcommand{\bbb}{\frac{b_1 + b_2}{b+b_1 + b_2 }}
\newcommand{\C}{C_{(q)}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\xlc}{X^{\text{LC}}}
\def\eqdef{\mathbin{:=}}
\def\Prob{{\sf P}}
\def\FRAC#1#2#3{\genfrac{}{}{}{#1}{#2}{#3}}

\def\ddx{\frac{\ud}{\ud x}}
\def\ddt{\frac{\ud}{\ud t}}
\def\J{{\sf J}}
\def\Jstar{J^*}  %I didn't like a simple "J" -spm
\newcommand{\ii}{k}

%\newcommand{\Xit}{\tilde{X}_t}
%\newcommand{\Xii}{\tilde{X}}
\newcommand{\Xii}{S}
\newcommand{\Eii}{\tilde{E}}
%\newcommand{\hatXit}{\hat{\tilde{X}}_t}
%\newcommand{\hatXii}{\hat{\tilde{X}}}
\newcommand{\hatXii}{\hat{S}}
\newcommand{\tn}{_{t_{n}}}
\newcommand{\tnn}{_{t_{n-1}}}
\newcommand{\Sigmaii}{\tilde{\Sigma}}
\def\kii{\tilde{\sf K}}
\newcommand{\var}{\text{Var}}
\newcommand{\X}{X}
\newcommand{\Om}{\Omega}
\newcommand{\NN}{\mathcal{N}}

\newcommand{\val}{\tilde{\phi}}
\newcommand{\phiN}{\phi^{(N)}}
\newcommand{\kepsnorm}{{k}^{(\epsilon)}}
\newcommand{\kepsnormN}{{k}^{(\epsilon,N)}}
\newcommand{\kepsnormNN}{\bar{k}^{(\epsilon,N_2)}}
\newcommand{\keps}{{k}_{\epsilon}}
\newcommand{\kepsN}{{k}_{\epsilon}^{(N)}}
\newcommand{\Keps}{{K}_\epsilon}
\newcommand{\KepsN}{{K}_\epsilon^{(N)}}
\newcommand{\Kepsnorm}{\bar{K}_\epsilon}
\newcommand{\KepsnormN}{\bar{K}_\epsilon^{(N)}}
\newcommand{\phiepsN}{{\phi}^{(N)}_\epsilon}
\newcommand{\phieps}{{\phi}_{\epsilon}}
\newcommand{\LepsN}{{L}_\epsilon^{(N)}}
\newcommand{\HH}{H^1_0}
\newcommand{\sumiN}{\sum_{i=1}^N}
\newcommand{\phiM}{\phi^{(M)}}
\newcommand{\phiMN}{\phi^{(M,N)}}
\newcommand{\Deltaeps}{{\Delta_\rho}^{(\epsilon)}}
\newcommand{\DeltaepsN}{{\Delta_\rho}^{(\epsilon,N)}}
\newcommand{\rhoepsN}{\rho^{(\epsilon,N)}}
\newcommand{\rhoeps}{\rho^{(\epsilon)}}
\newcommand{\Teps}{{T}_{\epsilon}}
\newcommand{\Aeps}{{A}^{(\epsilon)}}
\newcommand{\TepsN}{{T}^{(N)}_\epsilon}
\newcommand{\mueps}{{\mu}^{(\epsilon)}}
\newcommand{\geps}{{g}_{\epsilon}}
\newcommand{\pr}{\rho}
\newcommand{\neps}{{n}_\epsilon}
\newcommand{\nepsN}{{n}^{(N)}_\epsilon}
\newcommand{\Ltwoeps}{{L^2_0(\mueps)}}
\newcommand{\FF}{C_0(\Omega)}
\newcommand{\infnorm}[1]{\|#1\|_\infty}
\newcommand{\PhiepsN}{{\Phi}^{(\epsilon,N)}}
\newcommand{\vepsN}{{{\sf K}}_\epsilon^{(N)}}
%\floatname{algorithm}{Procedure}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\Geps}{{G}_\epsilon}
\newcommand{\GepsN}{{G}_\epsilon^{(N)}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\Km}{{\bf K}}
\newcommand{\hm}{{\bf h}}
\newcommand{\epsbar}{\bar{\epsilon}}
\newcommand{\meas}{\mu}
\newcommand{\aht}[1]{{\color{blue} \text{AHT: #1}}}
%\newcommand{N}{{T}^{(\epsilon,N_2)}}
%\newcommand{\Deltaeps}{\frac{1}{\epsilon}(I -e^{-\epsilon\Delta_\rho})}
\newcommand{\tf}{{t_f}}
\newcommand{\Hs}{a}
\newcommand{\sfJ}{{\sf J}}
